Truly Unordered Probabilistic Rule Sets for Multi-class Classification

Rule set learning has long been studied and has recently been frequently revisited due to the need for interpretable models. Still, existing methods have several shortcomings: 1) most recent methods require a binary feature matrix as input, while learning rules directly from numeric variables is understudied; 2) existing methods impose orders among rules, either explicitly or implicitly, which harms interpretability; and 3) currently no method exists for learning probabilistic rule sets for multi-class target variables (there is only one for probabilistic rule lists). We propose TURS, for Truly Unordered Rule Sets, which addresses these shortcomings. We first formalize the problem of learning truly unordered rule sets. To resolve conflicts caused by overlapping rules, i.e., instances covered by multiple rules, we propose a novel approach that exploits the probabilistic properties of our rule sets. We next develop a two-phase heuristic algorithm that learns rule sets by carefully growing rules. An important innovation is that we use a surrogate score to take the global potential of the rule set into account when learning a local rule. Finally, we empirically demonstrate that, compared to non-probabilistic and (explicitly or implicitly) ordered state-of-the-art methods, our method learns rule sets that not only have better interpretability but also better predictive performance.

==> datainfo.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{lrrrrr}
  \hline
data\_name & n & ncols & cat\_num\_cols & numerical\_num\_cols & num\_class \\ 
  \hline
anuran & 7195 &  24 &   0 &  23 &   4 \\ 
  avila & 20867 &  11 &   0 &  10 &  12 \\ 
  backnote & 1372 &   5 &   0 &   4 &   2 \\ 
  car & 1728 &   7 &   6 &   0 &   4 \\ 
  chess & 3196 &  37 &  36 &   0 &   2 \\ 
  contracept & 1473 &  10 &   7 &   2 &   3 \\ 
  diabetes & 768 &   9 &   0 &   8 &   2 \\ 
  ionosphere & 351 &  35 &   2 &  32 &   2 \\ 
  iris & 150 &   5 &   0 &   4 &   3 \\ 
  magic & 19020 &  11 &   0 &  10 &   2 \\ 
  tic-tac-toe & 958 &  10 &   9 &   0 &   2 \\ 
  waveform & 5000 &  22 &   0 &  21 &   3 \\ 
  wine & 178 &  14 &   0 &  13 &   3 \\ 
   \hline
\end{tabular}
\caption{Summary of datasets.}
\end{table}

==> exp2.tex <==
% Created by tikzDevice version 0.12.3.1 on 2022-04-05 11:38:26
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (341.50,139.1);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (341.50,139.1);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00,  0.00) rectangle (341.50,139.1);
\end{scope}
\begin{scope}
\path[clip] ( 34.16, 44.68) rectangle (341.40,139.04);
\definecolor{fillColor}{RGB}{255,255,255}

\path[fill=fillColor] ( 34.16, 44.68) rectangle (341.40,139.04);
\definecolor{drawColor}{gray}{0.92}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 34.16, 64.58) --
	(341.40, 64.58);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 34.16, 93.22) --
	(341.40, 93.22);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 34.16,121.86) --
	(341.40,121.86);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 34.16, 50.26) --
	(341.40, 50.26);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 34.16, 78.90) --
	(341.40, 78.90);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 34.16,107.54) --
	(341.40,107.54);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 34.16,136.18) --
	(341.40,136.18);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 48.12, 44.68) --
	( 48.12,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 71.40, 44.68) --
	( 71.40,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 94.67, 44.68) --
	( 94.67,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (117.95, 44.68) --
	(117.95,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (141.22, 44.68) --
	(141.22,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (164.50, 44.68) --
	(164.50,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (187.78, 44.68) --
	(187.78,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (211.05, 44.68) --
	(211.05,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (234.33, 44.68) --
	(234.33,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (257.60, 44.68) --
	(257.60,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (280.88, 44.68) --
	(280.88,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (304.15, 44.68) --
	(304.15,139.04);

\path[draw=drawColor,line width= 0.6pt,line join=round] (327.43, 44.68) --
	(327.43,139.04);
\definecolor{fillColor}{gray}{0.35}

\path[fill=fillColor] ( 37.65, 50.26) rectangle ( 58.60, 62.83);

\path[fill=fillColor] ( 60.92, 50.26) rectangle ( 81.87,134.75);

\path[fill=fillColor] ( 84.20, 50.26) rectangle (105.15, 67.90);

\path[fill=fillColor] (107.47, 50.26) rectangle (128.42, 78.50);

\path[fill=fillColor] (130.75, 50.26) rectangle (151.70, 61.63);

\path[fill=fillColor] (154.03, 50.26) rectangle (174.97, 60.66);

\path[fill=fillColor] (177.30, 50.26) rectangle (198.25, 64.29);

\path[fill=fillColor] (200.58, 48.97) rectangle (221.53, 50.26);

\path[fill=fillColor] (223.85, 49.60) rectangle (244.80, 50.26);

\path[fill=fillColor] (247.13, 50.26) rectangle (268.08, 78.01);

\path[fill=fillColor] (270.40, 50.26) rectangle (291.35,101.04);

\path[fill=fillColor] (293.68, 50.26) rectangle (314.63, 61.77);

\path[fill=fillColor] (316.96, 50.26) rectangle (337.90, 51.55);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round] ( 34.16, 44.68) rectangle (341.40,139.04);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (341.50,139.1);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 29.21, 47.23) {0.0};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 29.21, 75.87) {0.1};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 29.21,104.51) {0.2};

\node[text=drawColor,anchor=base east,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 29.21,133.15) {0.3};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (341.50,139.1);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 31.41, 50.26) --
	( 34.16, 50.26);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 31.41, 78.90) --
	( 34.16, 78.90);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 31.41,107.54) --
	( 34.16,107.54);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 31.41,136.18) --
	( 34.16,136.18);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (341.50,139.1);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 48.12, 41.93) --
	( 48.12, 44.68);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 71.40, 41.93) --
	( 71.40, 44.68);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 94.67, 41.93) --
	( 94.67, 44.68);

\path[draw=drawColor,line width= 0.6pt,line join=round] (117.95, 41.93) --
	(117.95, 44.68);

\path[draw=drawColor,line width= 0.6pt,line join=round] (141.22, 41.93) --
	(141.22, 44.68);

\path[draw=drawColor,line width= 0.6pt,line join=round] (164.50, 41.93) --
	(164.50, 44.68);

\path[draw=drawColor,line width= 0.6pt,line join=round] (187.78, 41.93) --
	(187.78, 44.68);

\path[draw=drawColor,line width= 0.6pt,line join=round] (211.05, 41.93) --
	(211.05, 44.68);

\path[draw=drawColor,line width= 0.6pt,line join=round] (234.33, 41.93) --
	(234.33, 44.68);

\path[draw=drawColor,line width= 0.6pt,line join=round] (257.60, 41.93) --
	(257.60, 44.68);

\path[draw=drawColor,line width= 0.6pt,line join=round] (280.88, 41.93) --
	(280.88, 44.68);

\path[draw=drawColor,line width= 0.6pt,line join=round] (304.15, 41.93) --
	(304.15, 44.68);

\path[draw=drawColor,line width= 0.6pt,line join=round] (327.43, 41.93) --
	(327.43, 44.68);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (341.50,139.1);
\definecolor{drawColor}{gray}{0.30}

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 51.12, 29.5) {anuran};

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 74.40, 29.5) {avila};

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 97.67, 29.5) {backnote};

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (120.95, 29.5) {car};

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (144.22, 29.5) {chess};

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (167.50, 29.5) {contracept};

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (190.78, 29.5) {diabetes};

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (214.05, 29.5) {ionosphere};

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (237.33, 29.5) {iris};

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (260.60, 29.5) {magic};

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (283.88, 29.5) {tic-tac-toe};

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (307.15, 29.5) {waveform};

\node[text=drawColor,rotate= 45.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (330.43, 29.5) {wine};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (341.50,139.1);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.9] at ( 13.08, 91.86) {AUC improvement};
\end{scope}
\end{tikzpicture}


==> numrules.tex <==
% \begin{table}[ht]
% \centering
% \begin{tabular}{lrrrrrrr}
%   \hline
% data & TURS & CN2 & BRS & DRS & CLASSY & RIPPER & CART \\ 
%   \hline
% backnote & 3.8 & 2.9 & 2.8 & 2.7 & 2.8 & 2.3 & 4.8 \\ 
%   contracept & 5.1 & 4.6 & --- & 4.9 & 2.2 & 3.5 & 12.5 \\ 
%   diabetes & 5.6 & 4.5 & 2.8 & 3.9 & 2.4 & 2.2 & 8.4 \\ 
%   iris & 2.3 & 2.1 & --- & 2.1 & 1.5 & 1.0 & 2.1 \\ 
%   tic-tac-toe & 5.1 & 3.7 & 3.0 & 3.9 & 3.1 & 5.3 & 7.8 \\ 
%   wine & 3.1 & 1.6 & --- & 4.2 & 2.8 & 1.8 & 2.7 \\ 
%   car & 5.4 & 3.8 & --- & 4.7 & 4.5 & 5.9 & 9.1 \\ 
%   anuran & 5.2 & 2.7 & --- & 9.3 & 3.4 & 1.7 & 4.9 \\ 
%   chess & 9.7 & 3.5 & 2.9 & 15.2 & 3.4 & 3.0 & 8.4 \\ 
%   ionosphere & 5.3 & 3.1 & 2.7 & 13.4 & 1.2 & 1.2 & 5.8 \\ 
%   waveform & 7.4 & 4.7 & --- & --- & 4.1 & 4.6 & 10.3 \\ 
%   avila & 6.8 & 3.5 & --- & 6.5 & 4.1 & 3.9 & 13.1 \\ 
%   magic & 7.9 & 4.8 & 3.0 & 3.6 & 3.6 & 3.3 & 15.6 \\ 
%   \hline
% \end{tabular}
% \end{table}

% \begin{table}[ht]
% \centering
% \begin{tabular}{lccccccc}
%   \hline
% data & TURS & CN2 & BRS & DRS & CLASSY & RIPPER & CART \\ 
%   \hline
% anuran & 14 & 4 & --- & 44 & 14 & 14 & 20 \\ 
%   avila & 130 & 147 & --- & 28 & 238 & 368 & 623 \\ 
%   backnote & 11 & 7 & 8 & 21 & 8 & 14 & 20 \\ 
%   car & 39 & 19 & --- & 70 & 20 & 42 & 79 \\ 
%   chess & 31 & 14 & 8 & 32 & 11 & 90 & 42 \\ 
%   contracept & 15 & 4 & --- & 15 & 7 & 60 & 499 \\ 
%   diabetes & 10 & 3 & 4 & 33 & 4 & 34 & 98 \\ 
%   ionosphere & 10 & 4 & 5 & 19 & 5 & 10 & 18 \\ 
%   iris & 3 & 3 & --- & 11 & 2 & 4 & 4 \\ 
%   magic & 168 & 21 & 8 & 13 & 70 & 464 & 1443 \\ 
%   tic-tac-toe & 17 & 11 & 8 & 27 & 9 & 24 & 105 \\ 
%   waveform & 96 & 25 & --- & 12 & 34 & 170 & 380 \\ 
%   wine & 3 & 3 & --- & 32 & 2 & 4 & 6 \\ 
%   \hline
% \end{tabular}
% \caption{Number of rules. Note that RIPPER only learns rules for $K-1$ classes for a $K$-class classification; and BRS only learns rules for the positive class for binary classification problem.}
% \end{table}
% \begin{table}[ht]
% \centering
% \begin{tabular}{lrrrrrr}
%   \hline
% data & CARS & RIPPER & CN2 & BRS & DRS & CART \\ 
%   \hline
% anuran & 14 & 4 & 14 & --- & --- & 20 \\ 
%   avila & 130 & 147 & 368 & --- & --- & 623 \\ 
%   backnote & 11 & 7 & 14 & 8 & 21 & 20 \\ 
%   car & 39 & 19 & 42 & --- & 70 & 79 \\ 
%   chess & 31 & 14 & 90 & 8 & 32 & 42 \\ 
%   contracept & 15 & 4 & 60 & --- & 15 & 499 \\ 
%   diabetes & 10 & 3 & 34 & 4 & 33 & 98 \\ 
%   ionosphere & 10 & 4 & 10 & 5 & 19 & 18 \\ 
%   iris & 3 & 3 & 4 & --- & 11 & 4 \\ 
%   magic & 168 & 21 & 464 & 8 & 13 & 1443 \\ 
%   tic-tac-toe & 17 & 11 & 24 & 8 & 27 & 105 \\ 
%   waveform & 96 & 25 & 170 & --- & 12 & 380 \\ 
%   wine & 3 & 3 & 4 & --- & 32 & 6 \\ 
%   \hline
% \end{tabular}
% \caption{Number of rules. Note that RIPPER only learns rules for $K-1$ classes for a $K$-class classification; and BRS only learns rules for the positive class for binary classification problem.}
% \end{table}
% \begin{table}[ht]
% \centering
% \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

%   \hline
% data &  \multicolumn{2}{c}{cars} &  \multicolumn{2}{|c|}{cn2} &  \multicolumn{2}{|c|}{BRS} &  \multicolumn{2}{|c|}{DRS} &  \multicolumn{2}{|c|}{CLASSY} &  \multicolumn{2}{|c|}{ripper} &  \multicolumn{2}{|c|}{CART} \\
% \hline
% &\# & len &\# & len &\# & len &\# & len &\# & len &\# & len &\# & len \\
% \hline
% anuran & 5.2 & 1.7 & -- & 9.3 & 3.4 & 2.7 & 4.9 & 14.4 & 4.1 & -- & 43.7 & 3.4 & 13.9 & 19.5 \\ 
%   avila & 6.8 & 3.9 & -- & 6.5 & 4.1 & 3.5 & 13.1 & 130.0 & 146.6 & -- & 27.7 & 4.1 & 368.1 & 622.6 \\ 
%   backnote & 3.8 & 2.3 & 2.8 & 2.7 & 2.8 & 2.9 & 4.8 & 11.1 & 7.1 & 7.7 & 20.6 & 2.8 & 14.1 & 19.7 \\ 
%   car & 5.4 & 5.9 & -- & 4.7 & 4.5 & 3.8 & 9.1 & 38.8 & 18.7 & -- & 69.7 & 4.5 & 42.4 & 78.8 \\ 
%   chess & 9.7 & 3.0 & 2.9 & 15.2 & 3.4 & 3.5 & 8.4 & 30.9 & 14.4 & 7.5 & 31.6 & 3.4 & 90.0 & 42.3 \\ 
%   contracept & 5.1 & 3.5 & -- & 4.9 & 2.2 & 4.6 & 12.5 & 14.7 & 4.2 & -- & 14.9 & 2.2 & 59.5 & 498.7 \\ 
%   diabetes & 5.6 & 2.2 & 2.8 & 3.9 & 2.4 & 4.5 & 8.4 & 9.7 & 2.7 & 3.7 & 33.1 & 2.4 & 33.9 & 98.5 \\ 
%   ionosphere & 5.3 & 1.2 & 2.7 & 13.4 & 1.2 & 3.1 & 5.8 & 9.5 & 4.0 & 5.3 & 19.4 & 1.2 & 9.6 & 17.6 \\ 
%   iris & 2.3 & 1.0 & -- & 2.1 & 1.5 & 2.1 & 2.1 & 3.2 & 2.9 & -- & 10.7 & 1.5 & 4.0 & 4.0 \\ 
%   magic & 7.9 & 3.3 & 3.0 & 3.6 & 3.6 & 4.8 & 15.6 & 167.7 & 20.9 & 7.8 & 13.1 & 3.6 & 464.0 & 1443.1 \\ 
%   tic-tac-toe & 5.1 & 5.3 & 3.0 & 3.9 & 3.1 & 3.7 & 7.8 & 17.1 & 11.3 & 8.0 & 27.4 & 3.1 & 24.4 & 104.9 \\ 
%   waveform & 7.4 & 4.6 & -- & -- & 4.1 & 4.7 & 10.3 & 95.8 & 25.1 & -- & 12.1 & 4.1 & 170.1 & 380.3 \\ 
%   wine & 3.1 & 1.8 & -- & 4.2 & 2.8 & 1.6 & 2.7 & 3.2 & 3.1 & -- & 32.3 & 2.8 & 4.0 & 5.8 \\ 
%   \hline
% \end{tabular}
% \end{table}
% \begin{table}[ht]
% \centering
% \begin{tabular}{lrrrrrrrrrrrrrr}
%   \hline
% data & cars & cn2 & BRS & DRS & CLASSY & ripper & CART & cars & cn2 & BRS & DRS & CLASSY & ripper & CART \\ 
%   \hline
% anuran & 5 & 2 & -- & 9 & 3 & 3 & 5 & 14 & 4 & -- & 44 & 3 & 14 & 20 \\ 
%   avila & 7 & 4 & -- & 6 & 4 & 4 & 13 & 130 & 147 & -- & 28 & 4 & 368 & 623 \\ 
%   backnote & 4 & 2 & 3 & 3 & 3 & 3 & 5 & 11 & 7 & 8 & 21 & 3 & 14 & 20 \\ 
%   car & 5 & 6 & -- & 5 & 4 & 4 & 9 & 39 & 19 & -- & 70 & 4 & 42 & 79 \\ 
%   chess & 10 & 3 & 3 & 15 & 3 & 4 & 8 & 31 & 14 & 8 & 32 & 3 & 90 & 42 \\ 
%   contracept & 5 & 3 & -- & 5 & 2 & 5 & 13 & 15 & 4 & -- & 15 & 2 & 60 & 499 \\ 
%   diabetes & 6 & 2 & 3 & 4 & 2 & 4 & 8 & 10 & 3 & 4 & 33 & 2 & 34 & 98 \\ 
%   ionosphere & 5 & 1 & 3 & 13 & 1 & 3 & 6 & 10 & 4 & 5 & 19 & 1 & 10 & 18 \\ 
%   iris & 2 & 1 & -- & 2 & 2 & 2 & 2 & 3 & 3 & -- & 11 & 2 & 4 & 4 \\ 
%   magic & 8 & 3 & 3 & 4 & 4 & 5 & 16 & 168 & 21 & 8 & 13 & 4 & 464 & 1443 \\ 
%   tic-tac-toe & 5 & 5 & 3 & 4 & 3 & 4 & 8 & 17 & 11 & 8 & 27 & 3 & 24 & 105 \\ 
%   waveform & 7 & 5 & -- & -- & 4 & 5 & 10 & 96 & 25 & -- & 12 & 4 & 170 & 380 \\ 
%   wine & 3 & 2 & -- & 4 & 3 & 2 & 3 & 3 & 3 & -- & 32 & 3 & 4 & 6 \\ 
%   \hline
% \end{tabular}
% \end{table}
